PortLLM: Personalizing Evolving Large Language Models with Training-Free and Portable Model Patches

As large language models (LLMs) increasingly shape the AI landscape, fine-tuning pretrained models has become more popular than in the pre-LLM era for achieving optimal performance in domain-specific tasks. However, pretrained LLMs such as ChatGPT are periodically evolved, i.e., model parameters are frequently updated), making it challenging for downstream users with limited resources to keep up with fine-tuning the newest LLMs for their domain application. Even though fine-tuning costs have nowadays been reduced thanks to the innovations of parameter-efficient fine-tuning such as LoRA, not all downstream users have adequate computing for frequent personalization. Moreover, access to fine-tuning datasets, particularly in sensitive domains such as healthcare, could be time-restrictive, making it crucial to retain the knowledge encoded in earlier fine-tuned rounds for future adaptation. In this paper, we present PortLLM, a training-free framework that (i) creates an initial lightweight model update patch to capture domain-specific knowledge, and (ii) allows a subsequent seamless plugging for the continual personalization of evolved LLM at minimal cost. Our extensive experiments cover seven representative datasets, from easier question-answering tasks {BoolQ, SST2} to harder reasoning tasks {WinoGrande, GSM8K}, and models including {Mistral-7B, Llama2, Llama3.1, and Gemma2}, validating the portability of our designed model patches and showcasing the effectiveness of our proposed framework. For instance, PortLLM achieves comparable performance to LoRA fine-tuning with reductions of up to 12.2x in GPU memory usage. Finally, we provide theoretical justifications to understand the portability of our model update patches, which offers new insights into the theoretical dimension of LLMs' personalization.

==> _derivation_bak.tex <==




\begin{subequations}
    \begin{align}
        \theta_i^\prime &= \theta_i + \Delta\theta + \underbrace{(\Delta \theta_i^\prime - \Delta\theta_i)}_{\text{Residual Matrix }C} \label{eq:pathway1-a} \\
        &=  \theta_i + \Delta\theta + C \\ 
        &= (\theta + \Delta \theta_i)+  \Delta \theta + C \\ 
        &= (\theta + \Delta \theta) + \Delta \theta_i + C \\ 
        &= \theta^\prime + \underbrace{\Delta\theta_i + C}_{\text{Model Patch}} \label{eq:pathway} \\
        &= \theta^\prime + \Delta\theta_i + \underbrace{U\Sigma V^T}_{\text{SVD of Residual Matrix}}
    \end{align}
    \label{eq:pathway1}
\end{subequations}
